Simulating quantum circuits with arbitrary local noise using Pauli Propagation

We present a polynomial-time classical algorithm for estimating expectation values of arbitrary observables on typical quantum circuits under any incoherent local noise, including non-unital or dephasing. Although previous research demonstrated that some carefully designed quantum circuits affected by non-unital noise cannot be efficiently simulated, we show that this does not apply to average-case circuits, as these can be efficiently simulated using Pauli-path methods. Specifically, we prove that, with high probability over the circuit gates choice, Pauli propagation algorithms with tailored truncation strategies achieve an inversely polynomially small simulation error. This result holds for arbitrary circuit topologies and for any local noise, under the assumption that the distribution of each circuit layer is invariant under single-qubit random gates. Under the same minimal assumptions, we also prove that most noisy circuits can be truncated to an effective logarithmic depth for the task of {estimating} expectation values of observables, thus generalizing prior results to a significantly broader class of circuit ensembles. We further numerically validate our algorithm with simulations on a $6\times6$ lattice of qubits under the effects of amplitude damping and dephasing noise, as well as real-time dynamics on an $11\times11$ lattice of qubits affected by amplitude damping.

==> commands.tex <==
% MISC

\newcommand{\diff}{\ensuremath\mathrm{d}}
\newcommand{\ddt}{\ensuremath{\frac{\diff}{\diff t}}}
\newcommand{\ppt}{\ensuremath{\frac{\partial}{\partial t}}}

\newcommand{\Id}{\ensuremath{\mathbb{I}}}

\newcommand{\e}{\ensuremath{\mathrm{e}}}
\newcommand{\kb}{\ensuremath{k_\mathrm{B}}}

\newcommand{\bangeq}{\ensuremath{\overset{!}{=}}}
\newcommand{\transp}{\ensuremath{\scriptscriptstyle T}}
\newcommand*{\pipe}{\ensuremath{\, | \, }}
%\newcommand*{\Tr}{\operatorname{Tr}}
\newcommand*{\conj}{\ensuremath{^{*}}}
\newcommand*{\dagg}{\ensuremath{^{\dagger}}}

% VECTORS

\newcommand{\opgrad}{\ensuremath{\nabla}}
\newcommand{\oprot}{\ensuremath{\nabla \times}}
\newcommand{\opdiv}{\ensuremath{\nabla}}

\providecommand{\myvec}[1]{\ensuremath{\boldsymbol{#1}}}




\makeatletter
\renewcommand{\@part}[1]{%
  \ifnum \c@secnumdepth >-1\relax
    \refstepcounter{part}%
  \fi
  \addcontentsline{toc}{part}{#1}%
  {\centering
   \interlinepenalty \@M
   \normalfont\Huge \bfseries #1\par}%
  \markboth{}{}}
\makeatother



\providecommand{\AA}{\ensuremath{\myvec{A}}}
\providecommand{\BB}{\ensuremath{\myvec{B}}}
\providecommand{\CC}{\ensuremath{\myvec{C}}}
\providecommand{\DD}{\ensuremath{\myvec{D}}}
\providecommand{\EE}{\ensuremath{\myvec{E}}}
\providecommand{\FF}{\ensuremath{\myvec{F}}}
\providecommand{\GG}{\ensuremath{\myvec{G}}}
\providecommand{\HH}{\ensuremath{\myvec{H}}}
\providecommand{\II}{\ensuremath{\myvec{I}}}
\providecommand{\JJ}{\ensuremath{\myvec{J}}}
\providecommand{\KK}{\ensuremath{\myvec{K}}}
\providecommand{\LL}{\ensuremath{\myvec{L}}}
\providecommand{\MM}{\ensuremath{\myvec{M}}}
\providecommand{\NN}{\ensuremath{\myvec{N}}}
\providecommand{\OO}{\ensuremath{\myvec{O}}}
\providecommand{\PP}{\ensuremath{\myvec{P}}}
\providecommand{\QQ}{\ensuremath{\myvec{Q}}}
\providecommand{\RR}{\ensuremath{\myvec{R}}}
\providecommand{\SS}{\ensuremath{\myvec{S}}}
\providecommand{\TT}{\ensuremath{\myvec{T}}}
\providecommand{\UU}{\ensuremath{\myvec{U}}}
\providecommand{\VV}{\ensuremath{\myvec{V}}}
\providecommand{\WW}{\ensuremath{\myvec{W}}}
\providecommand{\XX}{\ensuremath{\myvec{X}}}
\providecommand{\YY}{\ensuremath{\myvec{Y}}}
\providecommand{\ZZ}{\ensuremath{\myvec{Z}}}

\providecommand{\aa}{\ensuremath{\myvec{a}}}
\providecommand{\bb}{\ensuremath{\myvec{b}}}
\providecommand{\cc}{\ensuremath{\myvec{c}}}
\providecommand{\dd}{\ensuremath{\myvec{d}}}
\providecommand{\ee}{\ensuremath{\myvec{e}}}
\providecommand{\ff}{\ensuremath{\myvec{f}}}
\providecommand{\gg}{\ensuremath{\myvec{g}}}
\providecommand{\hh}{\ensuremath{\myvec{h}}}
\providecommand{\ii}{\ensuremath{\myvec{i}}}
\providecommand{\jj}{\ensuremath{\myvec{j}}}
\providecommand{\kk}{\ensuremath{\myvec{k}}}
\providecommand{\ll}{\ensuremath{\myvec{l}}}
\providecommand{\mm}{\ensuremath{\myvec{m}}}
\providecommand{\nn}{\ensuremath{\myvec{n}}}
\providecommand{\oo}{\ensuremath{\myvec{o}}}
\providecommand{\pp}{\ensuremath{\myvec{p}}}
\providecommand{\qq}{\ensuremath{\myvec{q}}}
\providecommand{\rr}{\ensuremath{\myvec{r}}}
\providecommand{\ss}{\ensuremath{\myvec{s}}}
\providecommand{\tt}{\ensuremath{\myvec{t}}}
\providecommand{\uu}{\ensuremath{\myvec{u}}}
\providecommand{\vv}{\ensuremath{\myvec{v}}}
\providecommand{\ww}{\ensuremath{\myvec{w}}}
\providecommand{\xx}{\ensuremath{\myvec{x}}}
\providecommand{\yy}{\ensuremath{\myvec{y}}}
\providecommand{\zz}{\ensuremath{\myvec{z}}}

\providecommand{\aalpha}{\ensuremath{\myvec{\alpha}}}
\providecommand{\bbeta}{\ensuremath{\myvec{\beta}}}
\providecommand{\ggamma}{\ensuremath{\myvec{\gamma}}}
\providecommand{\ddelta}{\ensuremath{\myvec{\delta}}}
\providecommand{\eepsilon}{\ensuremath{\myvec{\epsilon}}}
\providecommand{\vvarepsilon}{\ensuremath{\myvec{\varepsilon}}}
\providecommand{\zzeta}{\ensuremath{\myvec{\zeta}}}
\providecommand{\eeta}{\ensuremath{\myvec{\eta}}}
\providecommand{\ttheta}{\ensuremath{\myvec{\theta}}}
\providecommand{\vvartheta}{\ensuremath{\myvec{\vartheta}}}
\providecommand{\iiota}{\ensuremath{\myvec{\iota}}}
\providecommand{\kkappa}{\ensuremath{\myvec{\kappa}}}
\providecommand{\vvarkappa}{\ensuremath{\myvec{\varkappa}}}
\providecommand{\llambda}{\ensuremath{\myvec{\lambda}}}
\providecommand{\mmu}{\ensuremath{\myvec{\mu}}}
\providecommand{\nnu}{\ensuremath{\myvec{\nu}}}
\providecommand{\xxi}{\ensuremath{\myvec{\xi}}}
\providecommand{\oomicron}{\ensuremath{\myvec{\omicron}}}
\providecommand{\ppi}{\ensuremath{\myvec{\pi}}}
\providecommand{\vvarpi}{\ensuremath{\myvec{\varpi}}}
\providecommand{\rrho}{\ensuremath{\myvec{\rho}}}
\providecommand{\vvarrho}{\ensuremath{\myvec{\varrho}}}
\providecommand{\ssigma}{\ensuremath{\myvec{\sigma}}}
\providecommand{\vvarsigma}{\ensuremath{\myvec{\varsigma}}}
\providecommand{\ttau}{\ensuremath{\myvec{\tau}}}
\providecommand{\uupsilon}{\ensuremath{\myvec{\upsilon}}}
\providecommand{\pphi}{\ensuremath{\myvec{\phi}}}
\providecommand{\vvarphi}{\ensuremath{\myvec{\varphi}}}
\providecommand{\cchi}{\ensuremath{\myvec{\chi}}}
\providecommand{\ppsi}{\ensuremath{\myvec{\psi}}}
\providecommand{\oomega}{\ensuremath{\myvec{\omega}}}
\providecommand{\GGamma}{\ensuremath{\myvec{\Gamma}}}
\providecommand{\DDelta}{\ensuremath{\myvec{\Delta}}}
\providecommand{\TTheta}{\ensuremath{\myvec{\Theta}}}
\providecommand{\LLambda}{\ensuremath{\myvec{\Lambda}}}
\providecommand{\SSigma}{\ensuremath{\myvec{\Sigma}}}
\providecommand{\UUpsilon}{\ensuremath{\myvec{\Upsilon}}}
\providecommand{\PPhi}{\ensuremath{\myvec{\Phi}}}
\providecommand{\PPsi}{\ensuremath{\myvec{\Psi}}}
\providecommand{\OOmega}{\ensuremath{\myvec{\Omega}}}

% OPERATORS

\providecommand{\myop}[1]{\ensuremath{\hat{#1}}}

\providecommand{\opA}{\ensuremath{\myop{A}}}
\providecommand{\opB}{\ensuremath{\myop{B}}}
\providecommand{\opC}{\ensuremath{\myop{C}}}
\providecommand{\opD}{\ensuremath{\myop{D}}}
\providecommand{\opE}{\ensuremath{\myop{E}}}
\providecommand{\opF}{\ensuremath{\myop{F}}}
\providecommand{\opG}{\ensuremath{\myop{G}}}
\providecommand{\opH}{\ensuremath{\myop{H}}}
\providecommand{\opI}{\ensuremath{\myop{I}}}
\providecommand{\opJ}{\ensuremath{\myop{J}}}
\providecommand{\opK}{\ensuremath{\myop{K}}}
\providecommand{\opL}{\ensuremath{\myop{L}}}
\providecommand{\opM}{\ensuremath{\myop{M}}}
\providecommand{\opN}{\ensuremath{\myop{N}}}
\providecommand{\opO}{\ensuremath{\myop{O}}}
\providecommand{\opP}{\ensuremath{\myop{P}}}
\providecommand{\opQ}{\ensuremath{\myop{Q}}}
\providecommand{\opR}{\ensuremath{\myop{R}}}
\providecommand{\opS}{\ensuremath{\myop{S}}}
\providecommand{\opT}{\ensuremath{\myop{T}}}
\providecommand{\opU}{\ensuremath{\myop{U}}}
\providecommand{\opV}{\ensuremath{\myop{V}}}
\providecommand{\opW}{\ensuremath{\myop{W}}}
\providecommand{\opX}{\ensuremath{\myop{X}}}
\providecommand{\opY}{\ensuremath{\myop{Y}}}
\providecommand{\opZ}{\ensuremath{\myop{Z}}}

\providecommand{\opa}{\ensuremath{\myop{a}}}
\providecommand{\opb}{\ensuremath{\myop{b}}}
\providecommand{\opc}{\ensuremath{\myop{c}}}
\providecommand{\opd}{\ensuremath{\myop{d}}}
\providecommand{\ope}{\ensuremath{\myop{e}}}
\providecommand{\opf}{\ensuremath{\myop{f}}}
\providecommand{\opg}{\ensuremath{\myop{g}}}
\providecommand{\oph}{\ensuremath{\myop{h}}}
\providecommand{\opi}{\ensuremath{\myop{i}}}
\providecommand{\opj}{\ensuremath{\myop{j}}}
\providecommand{\opk}{\ensuremath{\myop{k}}}
\providecommand{\opl}{\ensuremath{\myop{l}}}
\providecommand{\opm}{\ensuremath{\myop{m}}}
\providecommand{\opn}{\ensuremath{\myop{n}}}
\providecommand{\opo}{\ensuremath{\myop{o}}}
\providecommand{\opp}{\ensuremath{\myop{p}}}
\providecommand{\opq}{\ensuremath{\myop{q}}}
\providecommand{\opr}{\ensuremath{\myop{r}}}
\providecommand{\ops}{\ensuremath{\myop{s}}}
\providecommand{\opt}{\ensuremath{\myop{t}}}
\providecommand{\opu}{\ensuremath{\myop{u}}}
\providecommand{\opv}{\ensuremath{\myop{v}}}
\providecommand{\opw}{\ensuremath{\myop{w}}}
\providecommand{\opx}{\ensuremath{\myop{x}}}
\providecommand{\opy}{\ensuremath{\myop{y}}}
\providecommand{\opz}{\ensuremath{\myop{z}}}

\providecommand{\opalpha}{\ensuremath{\myop{\alpha}}}
\providecommand{\opbeta}{\ensuremath{\myop{\beta}}}
\providecommand{\opgamma}{\ensuremath{\myop{\gamma}}}
\providecommand{\opdelta}{\ensuremath{\myop{\delta}}}
\providecommand{\opepsilon}{\ensuremath{\myop{\epsilon}}}
\providecommand{\opvarepsilon}{\ensuremath{\myop{\varepsilon}}}
\providecommand{\opzeta}{\ensuremath{\myop{\zeta}}}
\providecommand{\opeta}{\ensuremath{\myop{\eta}}}
\providecommand{\optheta}{\ensuremath{\myop{\theta}}}
\providecommand{\opvartheta}{\ensuremath{\myop{\vartheta}}}
\providecommand{\opiota}{\ensuremath{\myop{\iota}}}
\providecommand{\opkappa}{\ensuremath{\myop{\kappa}}}
\providecommand{\opvarkappa}{\ensuremath{\myop{\varkappa}}}
\providecommand{\oplambda}{\ensuremath{\myop{\lambda}}}
\providecommand{\opmu}{\ensuremath{\myop{\mu}}}
\providecommand{\opnu}{\ensuremath{\myop{\nu}}}
\providecommand{\opxi}{\ensuremath{\myop{\xi}}}
\providecommand{\opomicron}{\ensuremath{\myop{\omicron}}}
\providecommand{\oppi}{\ensuremath{\myop{\pi}}}
\providecommand{\opvarpi}{\ensuremath{\myop{\varpi}}}
\providecommand{\oprho}{\ensuremath{\myop{\rho}}}
\providecommand{\opvarrho}{\ensuremath{\myop{\varrho}}}
\providecommand{\opsigma}{\ensuremath{\myop{\sigma}}}
\providecommand{\opvarsigma}{\ensuremath{\myop{\varsigma}}}
\providecommand{\optau}{\ensuremath{\myop{\tau}}}
\providecommand{\opupsilon}{\ensuremath{\myop{\upsilon}}}
\providecommand{\opphi}{\ensuremath{\myop{\phi}}}
\providecommand{\opvarphi}{\ensuremath{\myop{\varphi}}}
\providecommand{\opchi}{\ensuremath{\myop{\chi}}}
\providecommand{\oppsi}{\ensuremath{\myop{\psi}}}
\providecommand{\opomega}{\ensuremath{\myop{\omega}}}
\providecommand{\opGamma}{\ensuremath{\myop{\Gamma}}}
\providecommand{\opDelta}{\ensuremath{\myop{\Delta}}}
\providecommand{\opTheta}{\ensuremath{\myop{\Theta}}}
\providecommand{\opLambda}{\ensuremath{\myop{\Lambda}}}
\providecommand{\opSigma}{\ensuremath{\myop{\Sigma}}}
\providecommand{\opUpsilon}{\ensuremath{\myop{\Upsilon}}}
\providecommand{\opPhi}{\ensuremath{\myop{\Phi}}}
\providecommand{\opPsi}{\ensuremath{\myop{\Psi}}}
\providecommand{\opOmega}{\ensuremath{\myop{\Omega}}}

\providecommand{\opAA}{\ensuremath{\myop{\myvec{A}}}}
\providecommand{\opBB}{\ensuremath{\myop{\myvec{B}}}}
\providecommand{\opCC}{\ensuremath{\myop{\myvec{C}}}}
\providecommand{\opDD}{\ensuremath{\myop{\myvec{D}}}}
\providecommand{\opEE}{\ensuremath{\myop{\myvec{E}}}}
\providecommand{\opFF}{\ensuremath{\myop{\myvec{F}}}}
\providecommand{\opGG}{\ensuremath{\myop{\myvec{G}}}}
\providecommand{\opHH}{\ensuremath{\myop{\myvec{H}}}}
\providecommand{\opII}{\ensuremath{\myop{\myvec{I}}}}
\providecommand{\opJJ}{\ensuremath{\myop{\myvec{J}}}}
\providecommand{\opKK}{\ensuremath{\myop{\myvec{K}}}}
\providecommand{\opLL}{\ensuremath{\myop{\myvec{L}}}}
\providecommand{\opMM}{\ensuremath{\myop{\myvec{M}}}}
\providecommand{\opNN}{\ensuremath{\myop{\myvec{N}}}}
\providecommand{\opOO}{\ensuremath{\myop{\myvec{O}}}}
\providecommand{\opPP}{\ensuremath{\myop{\myvec{P}}}}
\providecommand{\opQQ}{\ensuremath{\myop{\myvec{Q}}}}
\providecommand{\opRR}{\ensuremath{\myop{\myvec{R}}}}
\providecommand{\opSS}{\ensuremath{\myop{\myvec{S}}}}
\providecommand{\opTT}{\ensuremath{\myop{\myvec{T}}}}
\providecommand{\opUU}{\ensuremath{\myop{\myvec{U}}}}
\providecommand{\opVV}{\ensuremath{\myop{\myvec{V}}}}
\providecommand{\opWW}{\ensuremath{\myop{\myvec{W}}}}
\providecommand{\opXX}{\ensuremath{\myop{\myvec{X}}}}
\providecommand{\opYY}{\ensuremath{\myop{\myvec{Y}}}}
\providecommand{\opZZ}{\ensuremath{\myop{\myvec{Z}}}}
\providecommand{\opaa}{\ensuremath{\myop{\myvec{a}}}}
\providecommand{\opbb}{\ensuremath{\myop{\myvec{b}}}}
\providecommand{\opcc}{\ensuremath{\myop{\myvec{c}}}}
\providecommand{\opdd}{\ensuremath{\myop{\myvec{d}}}}
\providecommand{\opee}{\ensuremath{\myop{\myvec{e}}}}
\providecommand{\opff}{\ensuremath{\myop{\myvec{f}}}}
\providecommand{\opgg}{\ensuremath{\myop{\myvec{g}}}}
\providecommand{\ophh}{\ensuremath{\myop{\myvec{h}}}}
\providecommand{\opii}{\ensuremath{\myop{\myvec{i}}}}
\providecommand{\opjj}{\ensuremath{\myop{\myvec{j}}}}
\providecommand{\opkk}{\ensuremath{\myop{\myvec{k}}}}
\providecommand{\opll}{\ensuremath{\myop{\myvec{l}}}}
\providecommand{\opmm}{\ensuremath{\myop{\myvec{m}}}}
\providecommand{\opnn}{\ensuremath{\myop{\myvec{n}}}}
\providecommand{\opoo}{\ensuremath{\myop{\myvec{o}}}}
\providecommand{\oppp}{\ensuremath{\myop{\myvec{p}}}}
\providecommand{\opqq}{\ensuremath{\myop{\myvec{q}}}}
\providecommand{\oprr}{\ensuremath{\myop{\myvec{r}}}}
\providecommand{\opss}{\ensuremath{\myop{\myvec{s}}}}
\providecommand{\optt}{\ensuremath{\myop{\myvec{t}}}}
\providecommand{\opuu}{\ensuremath{\myop{\myvec{u}}}}
\providecommand{\opvv}{\ensuremath{\myop{\myvec{v}}}}
\providecommand{\opww}{\ensuremath{\myop{\myvec{w}}}}
\providecommand{\opxx}{\ensuremath{\myop{\myvec{x}}}}
\providecommand{\opyy}{\ensuremath{\myop{\myvec{y}}}}
\providecommand{\opzz}{\ensuremath{\myop{\myvec{z}}}}


\providecommand{\opAdag}{\ensuremath{\myop{A}^{\dagger}}}
\providecommand{\opBdag}{\ensuremath{\myop{B}^{\dagger}}}
\providecommand{\opCdag}{\ensuremath{\myop{C}^{\dagger}}}
\providecommand{\opDdag}{\ensuremath{\myop{D}^{\dagger}}}
\providecommand{\opEdag}{\ensuremath{\myop{E}^{\dagger}}}
\providecommand{\opFdag}{\ensuremath{\myop{F}^{\dagger}}}
\providecommand{\opGdag}{\ensuremath{\myop{G}^{\dagger}}}
\providecommand{\opHdag}{\ensuremath{\myop{H}^{\dagger}}}
\providecommand{\opIdag}{\ensuremath{\myop{I}^{\dagger}}}
\providecommand{\opJdag}{\ensuremath{\myop{J}^{\dagger}}}
\providecommand{\opKdag}{\ensuremath{\myop{K}^{\dagger}}}
\providecommand{\opLdag}{\ensuremath{\myop{L}^{\dagger}}}
\providecommand{\opMdag}{\ensuremath{\myop{M}^{\dagger}}}
\providecommand{\opNdag}{\ensuremath{\myop{N}^{\dagger}}}
\providecommand{\opOdag}{\ensuremath{\myop{O}^{\dagger}}}
\providecommand{\opPdag}{\ensuremath{\myop{P}^{\dagger}}}
\providecommand{\opQdag}{\ensuremath{\myop{Q}^{\dagger}}}
\providecommand{\opRdag}{\ensuremath{\myop{R}^{\dagger}}}
\providecommand{\opSdag}{\ensuremath{\myop{S}^{\dagger}}}
\providecommand{\opTdag}{\ensuremath{\myop{T}^{\dagger}}}
\providecommand{\opUdag}{\ensuremath{\myop{U}^{\dagger}}}
\providecommand{\opVdag}{\ensuremath{\myop{V}^{\dagger}}}
\providecommand{\opWdag}{\ensuremath{\myop{W}^{\dagger}}}
\providecommand{\opXdag}{\ensuremath{\myop{X}^{\dagger}}}
\providecommand{\opYdag}{\ensuremath{\myop{Y}^{\dagger}}}
\providecommand{\opZdag}{\ensuremath{\myop{Z}^{\dagger}}}

\providecommand{\opadag}{\ensuremath{\myop{a}^{\dagger}}}
\providecommand{\opbdag}{\ensuremath{\myop{b}^{\dagger}}}
\providecommand{\opcdag}{\ensuremath{\myop{c}^{\dagger}}}
\providecommand{\opddag}{\ensuremath{\myop{d}^{\dagger}}}
\providecommand{\opedag}{\ensuremath{\myop{e}^{\dagger}}}
\providecommand{\opfdag}{\ensuremath{\myop{f}^{\dagger}}}
\providecommand{\opgdag}{\ensuremath{\myop{g}^{\dagger}}}
\providecommand{\ophdag}{\ensuremath{\myop{h}^{\dagger}}}
\providecommand{\opidag}{\ensuremath{\myop{i}^{\dagger}}}
\providecommand{\opjdag}{\ensuremath{\myop{j}^{\dagger}}}
\providecommand{\opkdag}{\ensuremath{\myop{k}^{\dagger}}}
\providecommand{\opldag}{\ensuremath{\myop{l}^{\dagger}}}
\providecommand{\opmdag}{\ensuremath{\myop{m}^{\dagger}}}
\providecommand{\opndag}{\ensuremath{\myop{n}^{\dagger}}}
\providecommand{\opodag}{\ensuremath{\myop{o}^{\dagger}}}
\providecommand{\oppdag}{\ensuremath{\myop{p}^{\dagger}}}
\providecommand{\opqdag}{\ensuremath{\myop{q}^{\dagger}}}
\providecommand{\oprdag}{\ensuremath{\myop{r}^{\dagger}}}
\providecommand{\opsdag}{\ensuremath{\myop{s}^{\dagger}}}
\providecommand{\optdag}{\ensuremath{\myop{t}^{\dagger}}}
\providecommand{\opudag}{\ensuremath{\myop{u}^{\dagger}}}
\providecommand{\opvdag}{\ensuremath{\myop{v}^{\dagger}}}
\providecommand{\opwdag}{\ensuremath{\myop{w}^{\dagger}}}
\providecommand{\opxdag}{\ensuremath{\myop{x}^{\dagger}}}
\providecommand{\opydag}{\ensuremath{\myop{y}^{\dagger}}}
\providecommand{\opzdag}{\ensuremath{\myop{z}^{\dagger}}}

\providecommand{\opalphadag}{\ensuremath{\myop{\alpha}^{\dagger}}}
\providecommand{\opbetadag}{\ensuremath{\myop{\beta}^{\dagger}}}
\providecommand{\opgammadag}{\ensuremath{\myop{\gamma}^{\dagger}}}
\providecommand{\opdeltadag}{\ensuremath{\myop{\delta}^{\dagger}}}
\providecommand{\opepsilondag}{\ensuremath{\myop{\epsilon}^{\dagger}}}
\providecommand{\opvarepsilondag}{\ensuremath{\myop{\varepsilon}^{\dagger}}}
\providecommand{\opzetadag}{\ensuremath{\myop{\zeta}^{\dagger}}}
\providecommand{\opetadag}{\ensuremath{\myop{\eta}^{\dagger}}}
\providecommand{\opthetadag}{\ensuremath{\myop{\theta}^{\dagger}}}
\providecommand{\opvarthetadag}{\ensuremath{\myop{\vartheta}^{\dagger}}}
\providecommand{\opiotadag}{\ensuremath{\myop{\iota}^{\dagger}}}
\providecommand{\opkappadag}{\ensuremath{\myop{\kappa}^{\dagger}}}
\providecommand{\opvarkappadag}{\ensuremath{\myop{\varkappa}^{\dagger}}}
\providecommand{\oplambdadag}{\ensuremath{\myop{\lambda}^{\dagger}}}
\providecommand{\opmudag}{\ensuremath{\myop{\mu}^{\dagger}}}
\providecommand{\opnudag}{\ensuremath{\myop{\nu}^{\dagger}}}
\providecommand{\opxidag}{\ensuremath{\myop{\xi}^{\dagger}}}
\providecommand{\opomicrondag}{\ensuremath{\myop{\omicron}^{\dagger}}}
\providecommand{\oppidag}{\ensuremath{\myop{\pi}^{\dagger}}}
\providecommand{\opvarpidag}{\ensuremath{\myop{\varpi}^{\dagger}}}
\providecommand{\oprhodag}{\ensuremath{\myop{\rho}^{\dagger}}}
\providecommand{\opvarrhodag}{\ensuremath{\myop{\varrho}^{\dagger}}}
\providecommand{\opsigmadag}{\ensuremath{\myop{\sigma}^{\dagger}}}
\providecommand{\opvarsigmadag}{\ensuremath{\myop{\varsigma}^{\dagger}}}
\providecommand{\optaudag}{\ensuremath{\myop{\tau}^{\dagger}}}
\providecommand{\opupsilondag}{\ensuremath{\myop{\upsilon}^{\dagger}}}
\providecommand{\opphidag}{\ensuremath{\myop{\phi}^{\dagger}}}
\providecommand{\opvarphidag}{\ensuremath{\myop{\varphi}^{\dagger}}}
\providecommand{\opchidag}{\ensuremath{\myop{\chi}^{\dagger}}}
\providecommand{\oppsidag}{\ensuremath{\myop{\psi}^{\dagger}}}
\providecommand{\opomegadag}{\ensuremath{\myop{\omega}^{\dagger}}}
\providecommand{\opGammadag}{\ensuremath{\myop{\Gamma}^{\dagger}}}
\providecommand{\opDeltadag}{\ensuremath{\myop{\Delta}^{\dagger}}}
\providecommand{\opThetadag}{\ensuremath{\myop{\Theta}^{\dagger}}}
\providecommand{\opLambdadag}{\ensuremath{\myop{\Lambda}^{\dagger}}}
\providecommand{\opSigmadag}{\ensuremath{\myop{\Sigma}^{\dagger}}}
\providecommand{\opUpsilondag}{\ensuremath{\myop{\Upsilon}^{\dagger}}}
\providecommand{\opPhidag}{\ensuremath{\myop{\Phi}^{\dagger}}}
\providecommand{\opPsidag}{\ensuremath{\myop{\Psi}^{\dagger}}}
\providecommand{\opOmegadag}{\ensuremath{\myop{\Omega}^{\dagger}}}

\providecommand{\opAAdag}{\ensuremath{\myop{\myvec{A}}^{\dagger}}}
\providecommand{\opBBdag}{\ensuremath{\myop{\myvec{B}}^{\dagger}}}
\providecommand{\opCCdag}{\ensuremath{\myop{\myvec{C}}^{\dagger}}}
\providecommand{\opDDdag}{\ensuremath{\myop{\myvec{D}}^{\dagger}}}
\providecommand{\opEEdag}{\ensuremath{\myop{\myvec{E}}^{\dagger}}}
\providecommand{\opFFdag}{\ensuremath{\myop{\myvec{F}}^{\dagger}}}
\providecommand{\opGGdag}{\ensuremath{\myop{\myvec{G}}^{\dagger}}}
\providecommand{\opHHdag}{\ensuremath{\myop{\myvec{H}}^{\dagger}}}
\providecommand{\opIIdag}{\ensuremath{\myop{\myvec{I}}^{\dagger}}}
\providecommand{\opJJdag}{\ensuremath{\myop{\myvec{J}}^{\dagger}}}
\providecommand{\opKKdag}{\ensuremath{\myop{\myvec{K}}^{\dagger}}}
\providecommand{\opLLdag}{\ensuremath{\myop{\myvec{L}}^{\dagger}}}
\providecommand{\opMMdag}{\ensuremath{\myop{\myvec{M}}^{\dagger}}}
\providecommand{\opNNdag}{\ensuremath{\myop{\myvec{N}}^{\dagger}}}
\providecommand{\opOOdag}{\ensuremath{\myop{\myvec{O}}^{\dagger}}}
\providecommand{\opPPdag}{\ensuremath{\myop{\myvec{P}}^{\dagger}}}
\providecommand{\opQQdag}{\ensuremath{\myop{\myvec{Q}}^{\dagger}}}
\providecommand{\opRRdag}{\ensuremath{\myop{\myvec{R}}^{\dagger}}}
\providecommand{\opSSdag}{\ensuremath{\myop{\myvec{S}}^{\dagger}}}
\providecommand{\opTTdag}{\ensuremath{\myop{\myvec{T}}^{\dagger}}}
\providecommand{\opUUdag}{\ensuremath{\myop{\myvec{U}}^{\dagger}}}
\providecommand{\opVVdag}{\ensuremath{\myop{\myvec{V}}^{\dagger}}}
\providecommand{\opWWdag}{\ensuremath{\myop{\myvec{W}}^{\dagger}}}
\providecommand{\opXXdag}{\ensuremath{\myop{\myvec{X}}^{\dagger}}}
\providecommand{\opYYdag}{\ensuremath{\myop{\myvec{Y}}^{\dagger}}}
\providecommand{\opZZdag}{\ensuremath{\myop{\myvec{Z}}^{\dagger}}}
\providecommand{\opaadag}{\ensuremath{\myop{\myvec{a}}^{\dagger}}}
\providecommand{\opbbdag}{\ensuremath{\myop{\myvec{b}}^{\dagger}}}
\providecommand{\opccdag}{\ensuremath{\myop{\myvec{c}}^{\dagger}}}
\providecommand{\opdddag}{\ensuremath{\myop{\myvec{d}}^{\dagger}}}
\providecommand{\opeedag}{\ensuremath{\myop{\myvec{e}}^{\dagger}}}
\providecommand{\opffdag}{\ensuremath{\myop{\myvec{f}}^{\dagger}}}
\providecommand{\opggdag}{\ensuremath{\myop{\myvec{g}}^{\dagger}}}
\providecommand{\ophhdag}{\ensuremath{\myop{\myvec{h}}^{\dagger}}}
\providecommand{\opiidag}{\ensuremath{\myop{\myvec{i}}^{\dagger}}}
\providecommand{\opjjdag}{\ensuremath{\myop{\myvec{j}}^{\dagger}}}
\providecommand{\opkkdag}{\ensuremath{\myop{\myvec{k}}^{\dagger}}}
\providecommand{\oplldag}{\ensuremath{\myop{\myvec{l}}^{\dagger}}}
\providecommand{\opmmdag}{\ensuremath{\myop{\myvec{m}}^{\dagger}}}
\providecommand{\opnndag}{\ensuremath{\myop{\myvec{n}}^{\dagger}}}
\providecommand{\opoodag}{\ensuremath{\myop{\myvec{o}}^{\dagger}}}
\providecommand{\opppdag}{\ensuremath{\myop{\myvec{p}}^{\dagger}}}
\providecommand{\opqqdag}{\ensuremath{\myop{\myvec{q}}^{\dagger}}}
\providecommand{\oprrdag}{\ensuremath{\myop{\myvec{r}}^{\dagger}}}
\providecommand{\opssdag}{\ensuremath{\myop{\myvec{s}}^{\dagger}}}
\providecommand{\opttdag}{\ensuremath{\myop{\myvec{t}}^{\dagger}}}
\providecommand{\opuudag}{\ensuremath{\myop{\myvec{u}}^{\dagger}}}
\providecommand{\opvvdag}{\ensuremath{\myop{\myvec{v}}^{\dagger}}}
\providecommand{\opwwdag}{\ensuremath{\myop{\myvec{w}}^{\dagger}}}
\providecommand{\opxxdag}{\ensuremath{\myop{\myvec{x}}^{\dagger}}}
\providecommand{\opyydag}{\ensuremath{\myop{\myvec{y}}^{\dagger}}}
\providecommand{\opzzdag}{\ensuremath{\myop{\myvec{z}}^{\dagger}}}

% MATHCAL

\providecommand{\calA}{\ensuremath{\mathcal{A}}}
\providecommand{\calB}{\ensuremath{\mathcal{B}}}
\providecommand{\calC}{\ensuremath{\mathcal{C}}}
\providecommand{\calD}{\ensuremath{\mathcal{D}}}
\providecommand{\calE}{\ensuremath{\mathcal{E}}}
\providecommand{\calF}{\ensuremath{\mathcal{F}}}
\providecommand{\calG}{\ensuremath{\mathcal{G}}}
\providecommand{\calH}{\ensuremath{\mathcal{H}}}
\providecommand{\calI}{\ensuremath{\mathcal{I}}}
\providecommand{\calJ}{\ensuremath{\mathcal{J}}}
\providecommand{\calK}{\ensuremath{\mathcal{K}}}
\providecommand{\calL}{\ensuremath{\mathcal{L}}}
\providecommand{\calM}{\ensuremath{\mathcal{M}}}
\providecommand{\calN}{\ensuremath{\mathcal{N}}}
\providecommand{\calO}{\ensuremath{\mathcal{O}}}
\providecommand{\calP}{\ensuremath{\mathcal{P}}}
\providecommand{\calQ}{\ensuremath{\mathcal{Q}}}
\providecommand{\calR}{\ensuremath{\mathcal{R}}}
\providecommand{\calS}{\ensuremath{\mathcal{S}}}
\providecommand{\calT}{\ensuremath{\mathcal{T}}}
\providecommand{\calU}{\ensuremath{\mathcal{U}}}
\providecommand{\calV}{\ensuremath{\mathcal{V}}}
\providecommand{\calW}{\ensuremath{\mathcal{W}}}
\providecommand{\calX}{\ensuremath{\mathcal{X}}}
\providecommand{\calY}{\ensuremath{\mathcal{Y}}}
\providecommand{\calZ}{\ensuremath{\mathcal{Z}}}

\providecommand{\cala}{\ensuremath{\mathcal{a}}}
\providecommand{\calb}{\ensuremath{\mathcal{b}}}
\providecommand{\calc}{\ensuremath{\mathcal{c}}}
\providecommand{\cald}{\ensuremath{\mathcal{d}}}
\providecommand{\cale}{\ensuremath{\mathcal{e}}}
\providecommand{\calf}{\ensuremath{\mathcal{f}}}
\providecommand{\calg}{\ensuremath{\mathcal{g}}}
\providecommand{\calh}{\ensuremath{\mathcal{h}}}
\providecommand{\cali}{\ensuremath{\mathcal{i}}}
\providecommand{\calj}{\ensuremath{\mathcal{j}}}
\providecommand{\calk}{\ensuremath{\mathcal{k}}}
\providecommand{\call}{\ensuremath{\mathcal{l}}}
\providecommand{\calm}{\ensuremath{\mathcal{m}}}
\providecommand{\caln}{\ensuremath{\mathcal{n}}}
\providecommand{\calo}{\ensuremath{\mathcal{o}}}
\providecommand{\calp}{\ensuremath{\mathcal{p}}}
\providecommand{\calq}{\ensuremath{\mathcal{q}}}
\providecommand{\calr}{\ensuremath{\mathcal{r}}}
\providecommand{\cals}{\ensuremath{\mathcal{s}}}
\providecommand{\calt}{\ensuremath{\mathcal{t}}}
\providecommand{\calu}{\ensuremath{\mathcal{u}}}
\providecommand{\calv}{\ensuremath{\mathcal{v}}}
\providecommand{\calw}{\ensuremath{\mathcal{w}}}
\providecommand{\calx}{\ensuremath{\mathcal{x}}}
\providecommand{\caly}{\ensuremath{\mathcal{y}}}
\providecommand{\calz}{\ensuremath{\mathcal{z}}}

% MATHBB

\providecommand{\bbA}{\ensuremath{\mathbb{A}}}
\providecommand{\bbB}{\ensuremath{\mathbb{B}}}
\providecommand{\bbC}{\ensuremath{\mathbb{C}}}
\providecommand{\bbD}{\ensuremath{\mathbb{D}}}
\providecommand{\bbE}{\ensuremath{\mathbb{E}}}
\providecommand{\bbF}{\ensuremath{\mathbb{F}}}
\providecommand{\bbG}{\ensuremath{\mathbb{G}}}
\providecommand{\bbH}{\ensuremath{\mathbb{H}}}
\providecommand{\bbI}{\ensuremath{\mathbb{I}}}
\providecommand{\bbJ}{\ensuremath{\mathbb{J}}}
\providecommand{\bbK}{\ensuremath{\mathbb{K}}}
\providecommand{\bbL}{\ensuremath{\mathbb{L}}}
\providecommand{\bbM}{\ensuremath{\mathbb{M}}}
\providecommand{\bbN}{\ensuremath{\mathbb{N}}}
\providecommand{\bbO}{\ensuremath{\mathbb{O}}}
\providecommand{\bbP}{\ensuremath{\mathbb{P}}}
\providecommand{\bbQ}{\ensuremath{\mathbb{Q}}}
\providecommand{\bbR}{\ensuremath{\mathbb{R}}}
\providecommand{\bbS}{\ensuremath{\mathbb{S}}}
\providecommand{\bbT}{\ensuremath{\mathbb{T}}}
\providecommand{\bbU}{\ensuremath{\mathbb{U}}}
\providecommand{\bbV}{\ensuremath{\mathbb{V}}}
\providecommand{\bbW}{\ensuremath{\mathbb{W}}}
\providecommand{\bbX}{\ensuremath{\mathbb{X}}}
\providecommand{\bbY}{\ensuremath{\mathbb{Y}}}
\providecommand{\bbZ}{\ensuremath{\mathbb{Z}}}

% MATHFRAK

\providecommand{\frakA}{\ensuremath{\mathfrak{A}}}
\providecommand{\frakB}{\ensuremath{\mathfrak{B}}}
\providecommand{\frakC}{\ensuremath{\mathfrak{C}}}
\providecommand{\frakD}{\ensuremath{\mathfrak{D}}}
\providecommand{\frakE}{\ensuremath{\mathfrak{E}}}
\providecommand{\frakF}{\ensuremath{\mathfrak{F}}}
\providecommand{\frakG}{\ensuremath{\mathfrak{G}}}
\providecommand{\frakH}{\ensuremath{\mathfrak{H}}}
\providecommand{\frakI}{\ensuremath{\mathfrak{I}}}
\providecommand{\frakJ}{\ensuremath{\mathfrak{J}}}
\providecommand{\frakK}{\ensuremath{\mathfrak{K}}}
\providecommand{\frakL}{\ensuremath{\mathfrak{L}}}
\providecommand{\frakM}{\ensuremath{\mathfrak{M}}}
\providecommand{\frakN}{\ensuremath{\mathfrak{N}}}
\providecommand{\frakO}{\ensuremath{\mathfrak{O}}}
\providecommand{\frakP}{\ensuremath{\mathfrak{P}}}
\providecommand{\frakQ}{\ensuremath{\mathfrak{Q}}}
\providecommand{\frakR}{\ensuremath{\mathfrak{R}}}
\providecommand{\frakS}{\ensuremath{\mathfrak{S}}}
\providecommand{\frakT}{\ensuremath{\mathfrak{T}}}
\providecommand{\frakU}{\ensuremath{\mathfrak{U}}}
\providecommand{\frakV}{\ensuremath{\mathfrak{V}}}
\providecommand{\frakW}{\ensuremath{\mathfrak{W}}}
\providecommand{\frakX}{\ensuremath{\mathfrak{X}}}
\providecommand{\frakY}{\ensuremath{\mathfrak{Y}}}
\providecommand{\frakZ}{\ensuremath{\mathfrak{Z}}}
\providecommand{\fraka}{\ensuremath{\mathfrak{a}}}
\providecommand{\frakb}{\ensuremath{\mathfrak{b}}}
\providecommand{\frakc}{\ensuremath{\mathfrak{c}}}
\providecommand{\frakd}{\ensuremath{\mathfrak{d}}}
\providecommand{\frake}{\ensuremath{\mathfrak{e}}}
\providecommand{\frakf}{\ensuremath{\mathfrak{f}}}
\providecommand{\frakg}{\ensuremath{\mathfrak{g}}}
\providecommand{\frakh}{\ensuremath{\mathfrak{h}}}
\providecommand{\fraki}{\ensuremath{\mathfrak{i}}}
\providecommand{\frakj}{\ensuremath{\mathfrak{j}}}
\providecommand{\frakk}{\ensuremath{\mathfrak{k}}}
\providecommand{\frakl}{\ensuremath{\mathfrak{l}}}
\providecommand{\frakm}{\ensuremath{\mathfrak{m}}}
\providecommand{\frakn}{\ensuremath{\mathfrak{n}}}
\providecommand{\frako}{\ensuremath{\mathfrak{o}}}
\providecommand{\frakp}{\ensuremath{\mathfrak{p}}}
\providecommand{\frakq}{\ensuremath{\mathfrak{q}}}
\providecommand{\frakr}{\ensuremath{\mathfrak{r}}}
\providecommand{\fraks}{\ensuremath{\mathfrak{s}}}
\providecommand{\frakt}{\ensuremath{\mathfrak{t}}}
\providecommand{\fraku}{\ensuremath{\mathfrak{u}}}
\providecommand{\frakv}{\ensuremath{\mathfrak{v}}}
\providecommand{\frakw}{\ensuremath{\mathfrak{w}}}
\providecommand{\frakx}{\ensuremath{\mathfrak{x}}}
\providecommand{\fraky}{\ensuremath{\mathfrak{y}}}
\providecommand{\frakz}{\ensuremath{\mathfrak{z}}}

\providecommand{\DD}{\ensuremath{\myvec{D}}}
\providecommand{\EE}{\ensuremath{\myvec{E}}}
\providecommand{\FF}{\ensuremath{\myvec{F}}}
\providecommand{\GG}{\ensuremath{\myvec{G}}}
\providecommand{\HH}{\ensuremath{\myvec{H}}}
\providecommand{\II}{\ensuremath{\myvec{I}}}
\providecommand{\JJ}{\ensuremath{\myvec{J}}}
\providecommand{\KK}{\ensuremath{\myvec{K}}}
\providecommand{\LL}{\ensuremath{\myvec{L}}}
\providecommand{\MM}{\ensuremath{\myvec{M}}}
\providecommand{\NN}{\ensuremath{\myvec{N}}}
\providecommand{\OO}{\ensuremath{\myvec{O}}}
\providecommand{\PP}{\ensuremath{\myvec{P}}}
\providecommand{\QQ}{\ensuremath{\myvec{Q}}}
\providecommand{\RR}{\ensuremath{\myvec{R}}}
\providecommand{\SS}{\ensuremath{\myvec{S}}}
\providecommand{\TT}{\ensuremath{\myvec{T}}}
\providecommand{\UU}{\ensuremath{\myvec{U}}}
\providecommand{\VV}{\ensuremath{\myvec{V}}}
\providecommand{\WW}{\ensuremath{\myvec{W}}}
\providecommand{\XX}{\ensuremath{\myvec{X}}}
\providecommand{\YY}{\ensuremath{\myvec{Y}}}
\providecommand{\ZZ}{\ensuremath{\myvec{Z}}}

\providecommand{\aa}{\ensuremath{\myvec{a}}}
\providecommand{\bb}{\ensuremath{\myvec{b}}}
\providecommand{\cc}{\ensuremath{\myvec{c}}}
\providecommand{\dd}{\ensuremath{\myvec{d}}}
\providecommand{\ee}{\ensuremath{\myvec{e}}}
\providecommand{\ff}{\ensuremath{\myvec{f}}}
\providecommand{\gg}{\ensuremath{\myvec{g}}}
\providecommand{\hh}{\ensuremath{\myvec{h}}}
\providecommand{\ii}{\ensuremath{\myvec{i}}}
\providecommand{\jj}{\ensuremath{\myvec{j}}}
\providecommand{\kk}{\ensuremath{\myvec{k}}}
\providecommand{\ll}{\ensuremath{\myvec{l}}}
\providecommand{\mm}{\ensuremath{\myvec{m}}}
\providecommand{\nn}{\ensuremath{\myvec{n}}}
\providecommand{\oo}{\ensuremath{\myvec{o}}}
\providecommand{\pp}{\ensuremath{\myvec{p}}}
\providecommand{\qq}{\ensuremath{\myvec{q}}}
\providecommand{\rr}{\ensuremath{\myvec{r}}}
\providecommand{\ss}{\ensuremath{\myvec{s}}}
\providecommand{\tt}{\ensuremath{\myvec{t}}}
\providecommand{\uu}{\ensuremath{\myvec{u}}}
\providecommand{\vv}{\ensuremath{\myvec{v}}}
\providecommand{\ww}{\ensuremath{\myvec{w}}}
\providecommand{\xx}{\ensuremath{\myvec{x}}}
\providecommand{\yy}{\ensuremath{\myvec{y}}}
\providecommand{\zz}{\ensuremath{\myvec{z}}}

\providecommand{\aalpha}{\ensuremath{\myvec{\alpha}}}
\providecommand{\bbeta}{\ensuremath{\myvec{\beta}}}
\providecommand{\ggamma}{\ensuremath{\myvec{\gamma}}}
\providecommand{\ddelta}{\ensuremath{\myvec{\delta}}}
\providecommand{\eepsilon}{\ensuremath{\myvec{\epsilon}}}
\providecommand{\vvarepsilon}{\ensuremath{\myvec{\varepsilon}}}
\providecommand{\zzeta}{\ensuremath{\myvec{\zeta}}}
\providecommand{\eeta}{\ensuremath{\myvec{\eta}}}
\providecommand{\ttheta}{\ensuremath{\myvec{\theta}}}
\providecommand{\vvartheta}{\ensuremath{\myvec{\vartheta}}}
\providecommand{\iiota}{\ensuremath{\myvec{\iota}}}
\providecommand{\kkappa}{\ensuremath{\myvec{\kappa}}}
\providecommand{\vvarkappa}{\ensuremath{\myvec{\varkappa}}}
\providecommand{\llambda}{\ensuremath{\myvec{\lambda}}}
\providecommand{\mmu}{\ensuremath{\myvec{\mu}}}
\providecommand{\nnu}{\ensuremath{\myvec{\nu}}}
\providecommand{\xxi}{\ensuremath{\myvec{\xi}}}
\providecommand{\oomicron}{\ensuremath{\myvec{\omicron}}}
\providecommand{\ppi}{\ensuremath{\myvec{\pi}}}
\providecommand{\vvarpi}{\ensuremath{\myvec{\varpi}}}
\providecommand{\rrho}{\ensuremath{\myvec{\rho}}}
\providecommand{\vvarrho}{\ensuremath{\myvec{\varrho}}}
\providecommand{\ssigma}{\ensuremath{\myvec{\sigma}}}
\providecommand{\vvarsigma}{\ensuremath{\myvec{\varsigma}}}
\providecommand{\ttau}{\ensuremath{\myvec{\tau}}}
\providecommand{\uupsilon}{\ensuremath{\myvec{\upsilon}}}
\providecommand{\pphi}{\ensuremath{\myvec{\phi}}}
\providecommand{\vvarphi}{\ensuremath{\myvec{\varphi}}}
\providecommand{\cchi}{\ensuremath{\myvec{\chi}}}
\providecommand{\ppsi}{\ensuremath{\myvec{\psi}}}
\providecommand{\oomega}{\ensuremath{\myvec{\omega}}}
\providecommand{\GGamma}{\ensuremath{\myvec{\Gamma}}}
\providecommand{\DDelta}{\ensuremath{\myvec{\Delta}}}
\providecommand{\TTheta}{\ensuremath{\myvec{\Theta}}}
\providecommand{\LLambda}{\ensuremath{\myvec{\Lambda}}}
\providecommand{\SSigma}{\ensuremath{\myvec{\Sigma}}}
\providecommand{\UUpsilon}{\ensuremath{\myvec{\Upsilon}}}
\providecommand{\PPhi}{\ensuremath{\myvec{\Phi}}}
\providecommand{\PPsi}{\ensuremath{\myvec{\Psi}}}
\providecommand{\OOmega}{\ensuremath{\myvec{\Omega}}}

% OPERATORS

\providecommand{\myop}[1]{\ensuremath{\hat{#1}}}

\providecommand{\opA}{\ensuremath{\myop{A}}}
\providecommand{\opB}{\ensuremath{\myop{B}}}
\providecommand{\opC}{\ensuremath{\myop{C}}}
\providecommand{\opD}{\ensuremath{\myop{D}}}
\providecommand{\opE}{\ensuremath{\myop{E}}}
\providecommand{\opF}{\ensuremath{\myop{F}}}
\providecommand{\opG}{\ensuremath{\myop{G}}}
\providecommand{\opH}{\ensuremath{\myop{H}}}
\providecommand{\opI}{\ensuremath{\myop{I}}}
\providecommand{\opJ}{\ensuremath{\myop{J}}}
\providecommand{\opK}{\ensuremath{\myop{K}}}
\providecommand{\opL}{\ensuremath{\myop{L}}}
\providecommand{\opM}{\ensuremath{\myop{M}}}
\providecommand{\opN}{\ensuremath{\myop{N}}}
\providecommand{\opO}{\ensuremath{\myop{O}}}
\providecommand{\opP}{\ensuremath{\myop{P}}}
\providecommand{\opQ}{\ensuremath{\myop{Q}}}
\providecommand{\opR}{\ensuremath{\myop{R}}}
\providecommand{\opS}{\ensuremath{\myop{S}}}
\providecommand{\opT}{\ensuremath{\myop{T}}}
\providecommand{\opU}{\ensuremath{\myop{U}}}
\providecommand{\opV}{\ensuremath{\myop{V}}}
\providecommand{\opW}{\ensuremath{\myop{W}}}
\providecommand{\opX}{\ensuremath{\myop{X}}}
\providecommand{\opY}{\ensuremath{\myop{Y}}}
\providecommand{\opZ}{\ensuremath{\myop{Z}}}

\providecommand{\opa}{\ensuremath{\myop{a}}}
\providecommand{\opb}{\ensuremath{\myop{b}}}
\providecommand{\opc}{\ensuremath{\myop{c}}}
\providecommand{\opd}{\ensuremath{\myop{d}}}
\providecommand{\ope}{\ensuremath{\myop{e}}}
\providecommand{\opf}{\ensuremath{\myop{f}}}
\providecommand{\opg}{\ensuremath{\myop{g}}}
\providecommand{\oph}{\ensuremath{\myop{h}}}
\providecommand{\opi}{\ensuremath{\myop{i}}}
\providecommand{\opj}{\ensuremath{\myop{j}}}
\providecommand{\opk}{\ensuremath{\myop{k}}}
\providecommand{\opl}{\ensuremath{\myop{l}}}
\providecommand{\opm}{\ensuremath{\myop{m}}}
\providecommand{\opn}{\ensuremath{\myop{n}}}
\providecommand{\opo}{\ensuremath{\myop{o}}}
\providecommand{\opp}{\ensuremath{\myop{p}}}
\providecommand{\opq}{\ensuremath{\myop{q}}}
\providecommand{\opr}{\ensuremath{\myop{r}}}
\providecommand{\ops}{\ensuremath{\myop{s}}}
\providecommand{\opt}{\ensuremath{\myop{t}}}
\providecommand{\opu}{\ensuremath{\myop{u}}}
\providecommand{\opv}{\ensuremath{\myop{v}}}
\providecommand{\opw}{\ensuremath{\myop{w}}}
\providecommand{\opx}{\ensuremath{\myop{x}}}
\providecommand{\opy}{\ensuremath{\myop{y}}}
\providecommand{\opz}{\ensuremath{\myop{z}}}

\providecommand{\opalpha}{\ensuremath{\myop{\alpha}}}
\providecommand{\opbeta}{\ensuremath{\myop{\beta}}}
\providecommand{\opgamma}{\ensuremath{\myop{\gamma}}}
\providecommand{\opdelta}{\ensuremath{\myop{\delta}}}
\providecommand{\opepsilon}{\ensuremath{\myop{\epsilon}}}
\providecommand{\opvarepsilon}{\ensuremath{\myop{\varepsilon}}}
\providecommand{\opzeta}{\ensuremath{\myop{\zeta}}}
\providecommand{\opeta}{\ensuremath{\myop{\eta}}}
\providecommand{\optheta}{\ensuremath{\myop{\theta}}}
\providecommand{\opvartheta}{\ensuremath{\myop{\vartheta}}}
\providecommand{\opiota}{\ensuremath{\myop{\iota}}}
\providecommand{\opkappa}{\ensuremath{\myop{\kappa}}}
\providecommand{\opvarkappa}{\ensuremath{\myop{\varkappa}}}
\providecommand{\oplambda}{\ensuremath{\myop{\lambda}}}
\providecommand{\opmu}{\ensuremath{\myop{\mu}}}
\providecommand{\opnu}{\ensuremath{\myop{\nu}}}
\providecommand{\opxi}{\ensuremath{\myop{\xi}}}
\providecommand{\opomicron}{\ensuremath{\myop{\omicron}}}
\providecommand{\oppi}{\ensuremath{\myop{\pi}}}
\providecommand{\opvarpi}{\ensuremath{\myop{\varpi}}}
\providecommand{\oprho}{\ensuremath{\myop{\rho}}}
\providecommand{\opvarrho}{\ensuremath{\myop{\varrho}}}
\providecommand{\opsigma}{\ensuremath{\myop{\sigma}}}
\providecommand{\opvarsigma}{\ensuremath{\myop{\varsigma}}}
\providecommand{\optau}{\ensuremath{\myop{\tau}}}
\providecommand{\opupsilon}{\ensuremath{\myop{\upsilon}}}
\providecommand{\opphi}{\ensuremath{\myop{\phi}}}
\providecommand{\opvarphi}{\ensuremath{\myop{\varphi}}}
\providecommand{\opchi}{\ensuremath{\myop{\chi}}}
\providecommand{\oppsi}{\ensuremath{\myop{\psi}}}
\providecommand{\opomega}{\ensuremath{\myop{\omega}}}
\providecommand{\opGamma}{\ensuremath{\myop{\Gamma}}}
\providecommand{\opDelta}{\ensuremath{\myop{\Delta}}}
\providecommand{\opTheta}{\ensuremath{\myop{\Theta}}}
\providecommand{\opLambda}{\ensuremath{\myop{\Lambda}}}
\providecommand{\opSigma}{\ensuremath{\myop{\Sigma}}}
\providecommand{\opUpsilon}{\ensuremath{\myop{\Upsilon}}}
\providecommand{\opPhi}{\ensuremath{\myop{\Phi}}}
\providecommand{\opPsi}{\ensuremath{\myop{\Psi}}}
\providecommand{\opOmega}{\ensuremath{\myop{\Omega}}}

\providecommand{\opAA}{\ensuremath{\myop{\myvec{A}}}}
\providecommand{\opBB}{\ensuremath{\myop{\myvec{B}}}}
\providecommand{\opCC}{\ensuremath{\myop{\myvec{C}}}}
\providecommand{\opDD}{\ensuremath{\myop{\myvec{D}}}}
\providecommand{\opEE}{\ensuremath{\myop{\myvec{E}}}}
\providecommand{\opFF}{\ensuremath{\myop{\myvec{F}}}}
\providecommand{\opGG}{\ensuremath{\myop{\myvec{G}}}}
\providecommand{\opHH}{\ensuremath{\myop{\myvec{H}}}}
\providecommand{\opII}{\ensuremath{\myop{\myvec{I}}}}
\providecommand{\opJJ}{\ensuremath{\myop{\myvec{J}}}}
\providecommand{\opKK}{\ensuremath{\myop{\myvec{K}}}}
\providecommand{\opLL}{\ensuremath{\myop{\myvec{L}}}}
\providecommand{\opMM}{\ensuremath{\myop{\myvec{M}}}}
\providecommand{\opNN}{\ensuremath{\myop{\myvec{N}}}}
\providecommand{\opOO}{\ensuremath{\myop{\myvec{O}}}}
\providecommand{\opPP}{\ensuremath{\myop{\myvec{P}}}}
\providecommand{\opQQ}{\ensuremath{\myop{\myvec{Q}}}}
\providecommand{\opRR}{\ensuremath{\myop{\myvec{R}}}}
\providecommand{\opSS}{\ensuremath{\myop{\myvec{S}}}}
\providecommand{\opTT}{\ensuremath{\myop{\myvec{T}}}}
\providecommand{\opUU}{\ensuremath{\myop{\myvec{U}}}}
\providecommand{\opVV}{\ensuremath{\myop{\myvec{V}}}}
\providecommand{\opWW}{\ensuremath{\myop{\myvec{W}}}}
\providecommand{\opXX}{\ensuremath{\myop{\myvec{X}}}}
\providecommand{\opYY}{\ensuremath{\myop{\myvec{Y}}}}
\providecommand{\opZZ}{\ensuremath{\myop{\myvec{Z}}}}
\providecommand{\opaa}{\ensuremath{\myop{\myvec{a}}}}
\providecommand{\opbb}{\ensuremath{\myop{\myvec{b}}}}
\providecommand{\opcc}{\ensuremath{\myop{\myvec{c}}}}
\providecommand{\opdd}{\ensuremath{\myop{\myvec{d}}}}
\providecommand{\opee}{\ensuremath{\myop{\myvec{e}}}}
\providecommand{\opff}{\ensuremath{\myop{\myvec{f}}}}
\providecommand{\opgg}{\ensuremath{\myop{\myvec{g}}}}
\providecommand{\ophh}{\ensuremath{\myop{\myvec{h}}}}
\providecommand{\opii}{\ensuremath{\myop{\myvec{i}}}}
\providecommand{\opjj}{\ensuremath{\myop{\myvec{j}}}}
\providecommand{\opkk}{\ensuremath{\myop{\myvec{k}}}}
\providecommand{\opll}{\ensuremath{\myop{\myvec{l}}}}
\providecommand{\opmm}{\ensuremath{\myop{\myvec{m}}}}
\providecommand{\opnn}{\ensuremath{\myop{\myvec{n}}}}
\providecommand{\opoo}{\ensuremath{\myop{\myvec{o}}}}
\providecommand{\oppp}{\ensuremath{\myop{\myvec{p}}}}
\providecommand{\opqq}{\ensuremath{\myop{\myvec{q}}}}
\providecommand{\oprr}{\ensuremath{\myop{\myvec{r}}}}
\providecommand{\opss}{\ensuremath{\myop{\myvec{s}}}}
\providecommand{\optt}{\ensuremath{\myop{\myvec{t}}}}
\providecommand{\opuu}{\ensuremath{\myop{\myvec{u}}}}
\providecommand{\opvv}{\ensuremath{\myop{\myvec{v}}}}
\providecommand{\opww}{\ensuremath{\myop{\myvec{w}}}}
\providecommand{\opxx}{\ensuremath{\myop{\myvec{x}}}}
\providecommand{\opyy}{\ensuremath{\myop{\myvec{y}}}}
\providecommand{\opzz}{\ensuremath{\myop{\myvec{z}}}}


\providecommand{\opAdag}{\ensuremath{\myop{A}^{\dagger}}}
\providecommand{\opBdag}{\ensuremath{\myop{B}^{\dagger}}}
\providecommand{\opCdag}{\ensuremath{\myop{C}^{\dagger}}}
\providecommand{\opDdag}{\ensuremath{\myop{D}^{\dagger}}}
\providecommand{\opEdag}{\ensuremath{\myop{E}^{\dagger}}}
\providecommand{\opFdag}{\ensuremath{\myop{F}^{\dagger}}}
\providecommand{\opGdag}{\ensuremath{\myop{G}^{\dagger}}}
\providecommand{\opHdag}{\ensuremath{\myop{H}^{\dagger}}}
\providecommand{\opIdag}{\ensuremath{\myop{I}^{\dagger}}}
\providecommand{\opJdag}{\ensuremath{\myop{J}^{\dagger}}}
\providecommand{\opKdag}{\ensuremath{\myop{K}^{\dagger}}}
\providecommand{\opLdag}{\ensuremath{\myop{L}^{\dagger}}}
\providecommand{\opMdag}{\ensuremath{\myop{M}^{\dagger}}}
\providecommand{\opNdag}{\ensuremath{\myop{N}^{\dagger}}}
\providecommand{\opOdag}{\ensuremath{\myop{O}^{\dagger}}}
\providecommand{\opPdag}{\ensuremath{\myop{P}^{\dagger}}}
\providecommand{\opQdag}{\ensuremath{\myop{Q}^{\dagger}}}
\providecommand{\opRdag}{\ensuremath{\myop{R}^{\dagger}}}
\providecommand{\opSdag}{\ensuremath{\myop{S}^{\dagger}}}
\providecommand{\opTdag}{\ensuremath{\myop{T}^{\dagger}}}
\providecommand{\opUdag}{\ensuremath{\myop{U}^{\dagger}}}
\providecommand{\opVdag}{\ensuremath{\myop{V}^{\dagger}}}
\providecommand{\opWdag}{\ensuremath{\myop{W}^{\dagger}}}
\providecommand{\opXdag}{\ensuremath{\myop{X}^{\dagger}}}
\providecommand{\opYdag}{\ensuremath{\myop{Y}^{\dagger}}}
\providecommand{\opZdag}{\ensuremath{\myop{Z}^{\dagger}}}

\providecommand{\opadag}{\ensuremath{\myop{a}^{\dagger}}}
\providecommand{\opbdag}{\ensuremath{\myop{b}^{\dagger}}}
\providecommand{\opcdag}{\ensuremath{\myop{c}^{\dagger}}}
\providecommand{\opddag}{\ensuremath{\myop{d}^{\dagger}}}
\providecommand{\opedag}{\ensuremath{\myop{e}^{\dagger}}}
\providecommand{\opfdag}{\ensuremath{\myop{f}^{\dagger}}}
\providecommand{\opgdag}{\ensuremath{\myop{g}^{\dagger}}}
\providecommand{\ophdag}{\ensuremath{\myop{h}^{\dagger}}}
\providecommand{\opidag}{\ensuremath{\myop{i}^{\dagger}}}
\providecommand{\opjdag}{\ensuremath{\myop{j}^{\dagger}}}
\providecommand{\opkdag}{\ensuremath{\myop{k}^{\dagger}}}
\providecommand{\opldag}{\ensuremath{\myop{l}^{\dagger}}}
\providecommand{\opmdag}{\ensuremath{\myop{m}^{\dagger}}}
\providecommand{\opndag}{\ensuremath{\myop{n}^{\dagger}}}
\providecommand{\opodag}{\ensuremath{\myop{o}^{\dagger}}}
\providecommand{\oppdag}{\ensuremath{\myop{p}^{\dagger}}}
\providecommand{\opqdag}{\ensuremath{\myop{q}^{\dagger}}}
\providecommand{\oprdag}{\ensuremath{\myop{r}^{\dagger}}}
\providecommand{\opsdag}{\ensuremath{\myop{s}^{\dagger}}}
\providecommand{\optdag}{\ensuremath{\myop{t}^{\dagger}}}
\providecommand{\opudag}{\ensuremath{\myop{u}^{\dagger}}}
\providecommand{\opvdag}{\ensuremath{\myop{v}^{\dagger}}}
\providecommand{\opwdag}{\ensuremath{\myop{w}^{\dagger}}}
\providecommand{\opxdag}{\ensuremath{\myop{x}^{\dagger}}}
\providecommand{\opydag}{\ensuremath{\myop{y}^{\dagger}}}
\providecommand{\opzdag}{\ensuremath{\myop{z}^{\dagger}}}

\providecommand{\opalphadag}{\ensuremath{\myop{\alpha}^{\dagger}}}
\providecommand{\opbetadag}{\ensuremath{\myop{\beta}^{\dagger}}}
\providecommand{\opgammadag}{\ensuremath{\myop{\gamma}^{\dagger}}}
\providecommand{\opdeltadag}{\ensuremath{\myop{\delta}^{\dagger}}}
\providecommand{\opepsilondag}{\ensuremath{\myop{\epsilon}^{\dagger}}}
\providecommand{\opvarepsilondag}{\ensuremath{\myop{\varepsilon}^{\dagger}}}
\providecommand{\opzetadag}{\ensuremath{\myop{\zeta}^{\dagger}}}
\providecommand{\opetadag}{\ensuremath{\myop{\eta}^{\dagger}}}
\providecommand{\opthetadag}{\ensuremath{\myop{\theta}^{\dagger}}}
\providecommand{\opvarthetadag}{\ensuremath{\myop{\vartheta}^{\dagger}}}
\providecommand{\opiotadag}{\ensuremath{\myop{\iota}^{\dagger}}}
\providecommand{\opkappadag}{\ensuremath{\myop{\kappa}^{\dagger}}}
\providecommand{\opvarkappadag}{\ensuremath{\myop{\varkappa}^{\dagger}}}
\providecommand{\oplambdadag}{\ensuremath{\myop{\lambda}^{\dagger}}}
\providecommand{\opmudag}{\ensuremath{\myop{\mu}^{\dagger}}}
\providecommand{\opnudag}{\ensuremath{\myop{\nu}^{\dagger}}}
\providecommand{\opxidag}{\ensuremath{\myop{\xi}^{\dagger}}}
\providecommand{\opomicrondag}{\ensuremath{\myop{\omicron}^{\dagger}}}
\providecommand{\oppidag}{\ensuremath{\myop{\pi}^{\dagger}}}
\providecommand{\opvarpidag}{\ensuremath{\myop{\varpi}^{\dagger}}}
\providecommand{\oprhodag}{\ensuremath{\myop{\rho}^{\dagger}}}
\providecommand{\opvarrhodag}{\ensuremath{\myop{\varrho}^{\dagger}}}
\providecommand{\opsigmadag}{\ensuremath{\myop{\sigma}^{\dagger}}}
\providecommand{\opvarsigmadag}{\ensuremath{\myop{\varsigma}^{\dagger}}}
\providecommand{\optaudag}{\ensuremath{\myop{\tau}^{\dagger}}}
\providecommand{\opupsilondag}{\ensuremath{\myop{\upsilon}^{\dagger}}}
\providecommand{\opphidag}{\ensuremath{\myop{\phi}^{\dagger}}}
\providecommand{\opvarphidag}{\ensuremath{\myop{\varphi}^{\dagger}}}
\providecommand{\opchidag}{\ensuremath{\myop{\chi}^{\dagger}}}
\providecommand{\oppsidag}{\ensuremath{\myop{\psi}^{\dagger}}}
\providecommand{\opomegadag}{\ensuremath{\myop{\omega}^{\dagger}}}
\providecommand{\opGammadag}{\ensuremath{\myop{\Gamma}^{\dagger}}}
\providecommand{\opDeltadag}{\ensuremath{\myop{\Delta}^{\dagger}}}
\providecommand{\opThetadag}{\ensuremath{\myop{\Theta}^{\dagger}}}
\providecommand{\opLambdadag}{\ensuremath{\myop{\Lambda}^{\dagger}}}
\providecommand{\opSigmadag}{\ensuremath{\myop{\Sigma}^{\dagger}}}
\providecommand{\opUpsilondag}{\ensuremath{\myop{\Upsilon}^{\dagger}}}
\providecommand{\opPhidag}{\ensuremath{\myop{\Phi}^{\dagger}}}
\providecommand{\opPsidag}{\ensuremath{\myop{\Psi}^{\dagger}}}
\providecommand{\opOmegadag}{\ensuremath{\myop{\Omega}^{\dagger}}}

\providecommand{\opAAdag}{\ensuremath{\myop{\myvec{A}}^{\dagger}}}
\providecommand{\opBBdag}{\ensuremath{\myop{\myvec{B}}^{\dagger}}}
\providecommand{\opCCdag}{\ensuremath{\myop{\myvec{C}}^{\dagger}}}
\providecommand{\opDDdag}{\ensuremath{\myop{\myvec{D}}^{\dagger}}}
\providecommand{\opEEdag}{\ensuremath{\myop{\myvec{E}}^{\dagger}}}
\providecommand{\opFFdag}{\ensuremath{\myop{\myvec{F}}^{\dagger}}}
\providecommand{\opGGdag}{\ensuremath{\myop{\myvec{G}}^{\dagger}}}
\providecommand{\opHHdag}{\ensuremath{\myop{\myvec{H}}^{\dagger}}}
\providecommand{\opIIdag}{\ensuremath{\myop{\myvec{I}}^{\dagger}}}
\providecommand{\opJJdag}{\ensuremath{\myop{\myvec{J}}^{\dagger}}}
\providecommand{\opKKdag}{\ensuremath{\myop{\myvec{K}}^{\dagger}}}
\providecommand{\opLLdag}{\ensuremath{\myop{\myvec{L}}^{\dagger}}}
\providecommand{\opMMdag}{\ensuremath{\myop{\myvec{M}}^{\dagger}}}
\providecommand{\opNNdag}{\ensuremath{\myop{\myvec{N}}^{\dagger}}}
\providecommand{\opOOdag}{\ensuremath{\myop{\myvec{O}}^{\dagger}}}
\providecommand{\opPPdag}{\ensuremath{\myop{\myvec{P}}^{\dagger}}}
\providecommand{\opQQdag}{\ensuremath{\myop{\myvec{Q}}^{\dagger}}}
\providecommand{\opRRdag}{\ensuremath{\myop{\myvec{R}}^{\dagger}}}
\providecommand{\opSSdag}{\ensuremath{\myop{\myvec{S}}^{\dagger}}}
\providecommand{\opTTdag}{\ensuremath{\myop{\myvec{T}}^{\dagger}}}
\providecommand{\opUUdag}{\ensuremath{\myop{\myvec{U}}^{\dagger}}}
\providecommand{\opVVdag}{\ensuremath{\myop{\myvec{V}}^{\dagger}}}
\providecommand{\opWWdag}{\ensuremath{\myop{\myvec{W}}^{\dagger}}}
\providecommand{\opXXdag}{\ensuremath{\myop{\myvec{X}}^{\dagger}}}
\providecommand{\opYYdag}{\ensuremath{\myop{\myvec{Y}}^{\dagger}}}
\providecommand{\opZZdag}{\ensuremath{\myop{\myvec{Z}}^{\dagger}}}
\providecommand{\opaadag}{\ensuremath{\myop{\myvec{a}}^{\dagger}}}
\providecommand{\opbbdag}{\ensuremath{\myop{\myvec{b}}^{\dagger}}}
\providecommand{\opccdag}{\ensuremath{\myop{\myvec{c}}^{\dagger}}}
\providecommand{\opdddag}{\ensuremath{\myop{\myvec{d}}^{\dagger}}}
\providecommand{\opeedag}{\ensuremath{\myop{\myvec{e}}^{\dagger}}}
\providecommand{\opffdag}{\ensuremath{\myop{\myvec{f}}^{\dagger}}}
\providecommand{\opggdag}{\ensuremath{\myop{\myvec{g}}^{\dagger}}}
\providecommand{\ophhdag}{\ensuremath{\myop{\myvec{h}}^{\dagger}}}
\providecommand{\opiidag}{\ensuremath{\myop{\myvec{i}}^{\dagger}}}
\providecommand{\opjjdag}{\ensuremath{\myop{\myvec{j}}^{\dagger}}}
\providecommand{\opkkdag}{\ensuremath{\myop{\myvec{k}}^{\dagger}}}
\providecommand{\oplldag}{\ensuremath{\myop{\myvec{l}}^{\dagger}}}
\providecommand{\opmmdag}{\ensuremath{\myop{\myvec{m}}^{\dagger}}}
\providecommand{\opnndag}{\ensuremath{\myop{\myvec{n}}^{\dagger}}}
\providecommand{\opoodag}{\ensuremath{\myop{\myvec{o}}^{\dagger}}}
\providecommand{\opppdag}{\ensuremath{\myop{\myvec{p}}^{\dagger}}}
\providecommand{\opqqdag}{\ensuremath{\myop{\myvec{q}}^{\dagger}}}
\providecommand{\oprrdag}{\ensuremath{\myop{\myvec{r}}^{\dagger}}}
\providecommand{\opssdag}{\ensuremath{\myop{\myvec{s}}^{\dagger}}}
\providecommand{\opttdag}{\ensuremath{\myop{\myvec{t}}^{\dagger}}}
\providecommand{\opuudag}{\ensuremath{\myop{\myvec{u}}^{\dagger}}}
\providecommand{\opvvdag}{\ensuremath{\myop{\myvec{v}}^{\dagger}}}
\providecommand{\opwwdag}{\ensuremath{\myop{\myvec{w}}^{\dagger}}}
\providecommand{\opxxdag}{\ensuremath{\myop{\myvec{x}}^{\dagger}}}
\providecommand{\opyydag}{\ensuremath{\myop{\myvec{y}}^{\dagger}}}
\providecommand{\opzzdag}{\ensuremath{\myop{\myvec{z}}^{\dagger}}}

% MATHCAL

\providecommand{\calA}{\ensuremath{\mathcal{A}}}
\providecommand{\calB}{\ensuremath{\mathcal{B}}}
\providecommand{\calC}{\ensuremath{\mathcal{C}}}
\providecommand{\calD}{\ensuremath{\mathcal{D}}}
\providecommand{\calE}{\ensuremath{\mathcal{E}}}
\providecommand{\calF}{\ensuremath{\mathcal{F}}}
\providecommand{\calG}{\ensuremath{\mathcal{G}}}
\providecommand{\calH}{\ensuremath{\mathcal{H}}}
\providecommand{\calI}{\ensuremath{\mathcal{I}}}
\providecommand{\calJ}{\ensuremath{\mathcal{J}}}
\providecommand{\calK}{\ensuremath{\mathcal{K}}}
\providecommand{\calL}{\ensuremath{\mathcal{L}}}
\providecommand{\calM}{\ensuremath{\mathcal{M}}}
\providecommand{\calN}{\ensuremath{\mathcal{N}}}
\providecommand{\N}{\ensuremath{\mathcal{N}}}
\providecommand{\calO}{\ensuremath{\mathcal{O}}}
\providecommand{\calP}{\ensuremath{\mathcal{P}}}
\providecommand{\calQ}{\ensuremath{\mathcal{Q}}}
\providecommand{\calR}{\ensuremath{\mathcal{R}}}
\providecommand{\calS}{\ensuremath{\mathcal{S}}}
\providecommand{\calT}{\ensuremath{\mathcal{T}}}
\providecommand{\calU}{\ensuremath{\mathcal{U}}}
\providecommand{\calV}{\ensuremath{\mathcal{V}}}
\providecommand{\calW}{\ensuremath{\mathcal{W}}}
\providecommand{\calX}{\ensuremath{\mathcal{X}}}
\providecommand{\calY}{\ensuremath{\mathcal{Y}}}
\providecommand{\calZ}{\ensuremath{\mathcal{Z}}}

\providecommand{\cala}{\ensuremath{\mathcal{a}}}
\providecommand{\calb}{\ensuremath{\mathcal{b}}}
\providecommand{\calc}{\ensuremath{\mathcal{c}}}
\providecommand{\cald}{\ensuremath{\mathcal{d}}}
\providecommand{\cale}{\ensuremath{\mathcal{e}}}
\providecommand{\calf}{\ensuremath{\mathcal{f}}}
\providecommand{\calg}{\ensuremath{\mathcal{g}}}
\providecommand{\calh}{\ensuremath{\mathcal{h}}}
\providecommand{\cali}{\ensuremath{\mathcal{i}}}
\providecommand{\calj}{\ensuremath{\mathcal{j}}}
\providecommand{\calk}{\ensuremath{\mathcal{k}}}
\providecommand{\call}{\ensuremath{\mathcal{l}}}
\providecommand{\calm}{\ensuremath{\mathcal{m}}}
\providecommand{\caln}{\ensuremath{\mathcal{n}}}
\providecommand{\calo}{\ensuremath{\mathcal{o}}}
\providecommand{\calp}{\ensuremath{\mathcal{p}}}
\providecommand{\calq}{\ensuremath{\mathcal{q}}}
\providecommand{\calr}{\ensuremath{\mathcal{r}}}
\providecommand{\cals}{\ensuremath{\mathcal{s}}}
\providecommand{\calt}{\ensuremath{\mathcal{t}}}
\providecommand{\calu}{\ensuremath{\mathcal{u}}}
\providecommand{\calv}{\ensuremath{\mathcal{v}}}
\providecommand{\calw}{\ensuremath{\mathcal{w}}}
\providecommand{\calx}{\ensuremath{\mathcal{x}}}
\providecommand{\caly}{\ensuremath{\mathcal{y}}}
\providecommand{\calz}{\ensuremath{\mathcal{z}}}

% MATHBB

\providecommand{\bbA}{\ensuremath{\mathbb{A}}}
\providecommand{\bbB}{\ensuremath{\mathbb{B}}}
\providecommand{\bbC}{\ensuremath{\mathbb{C}}}
\providecommand{\bbD}{\ensuremath{\mathbb{D}}}
\providecommand{\bbE}{\ensuremath{\mathbb{E}}}
\providecommand{\bbF}{\ensuremath{\mathbb{F}}}
\providecommand{\bbG}{\ensuremath{\mathbb{G}}}
\providecommand{\bbH}{\ensuremath{\mathbb{H}}}
\providecommand{\bbI}{\ensuremath{\mathbb{I}}}
\providecommand{\bbJ}{\ensuremath{\mathbb{J}}}
\providecommand{\bbK}{\ensuremath{\mathbb{K}}}
\providecommand{\bbL}{\ensuremath{\mathbb{L}}}
\providecommand{\bbM}{\ensuremath{\mathbb{M}}}
\providecommand{\bbN}{\ensuremath{\mathbb{N}}}
\providecommand{\bbO}{\ensuremath{\mathbb{O}}}
\providecommand{\bbP}{\ensuremath{\mathbb{P}}}
\providecommand{\bbQ}{\ensuremath{\mathbb{Q}}}
\providecommand{\bbR}{\ensuremath{\mathbb{R}}}
\providecommand{\bbS}{\ensuremath{\mathbb{S}}}
\providecommand{\bbT}{\ensuremath{\mathbb{T}}}
\providecommand{\bbU}{\ensuremath{\mathbb{U}}}
\providecommand{\bbV}{\ensuremath{\mathbb{V}}}
\providecommand{\bbW}{\ensuremath{\mathbb{W}}}
\providecommand{\bbX}{\ensuremath{\mathbb{X}}}
\providecommand{\bbY}{\ensuremath{\mathbb{Y}}}
\providecommand{\bbZ}{\ensuremath{\mathbb{Z}}}

% MATHFRAK

\providecommand{\frakA}{\ensuremath{\mathfrak{A}}}
\providecommand{\frakB}{\ensuremath{\mathfrak{B}}}
\providecommand{\frakC}{\ensuremath{\mathfrak{C}}}
\providecommand{\frakD}{\ensuremath{\mathfrak{D}}}
\providecommand{\frakE}{\ensuremath{\mathfrak{E}}}
\providecommand{\frakF}{\ensuremath{\mathfrak{F}}}
\providecommand{\frakG}{\ensuremath{\mathfrak{G}}}
\providecommand{\frakH}{\ensuremath{\mathfrak{H}}}
\providecommand{\frakI}{\ensuremath{\mathfrak{I}}}
\providecommand{\frakJ}{\ensuremath{\mathfrak{J}}}
\providecommand{\frakK}{\ensuremath{\mathfrak{K}}}
\providecommand{\frakL}{\ensuremath{\mathfrak{L}}}
\providecommand{\frakM}{\ensuremath{\mathfrak{M}}}
\providecommand{\frakN}{\ensuremath{\mathfrak{N}}}
\providecommand{\frakO}{\ensuremath{\mathfrak{O}}}
\providecommand{\frakP}{\ensuremath{\mathfrak{P}}}
\providecommand{\frakQ}{\ensuremath{\mathfrak{Q}}}
\providecommand{\frakR}{\ensuremath{\mathfrak{R}}}
\providecommand{\frakS}{\ensuremath{\mathfrak{S}}}
\providecommand{\frakT}{\ensuremath{\mathfrak{T}}}
\providecommand{\frakU}{\ensuremath{\mathfrak{U}}}
\providecommand{\frakV}{\ensuremath{\mathfrak{V}}}
\providecommand{\frakW}{\ensuremath{\mathfrak{W}}}
\providecommand{\frakX}{\ensuremath{\mathfrak{X}}}
\providecommand{\frakY}{\ensuremath{\mathfrak{Y}}}
\providecommand{\frakZ}{\ensuremath{\mathfrak{Z}}}
\providecommand{\fraka}{\ensuremath{\mathfrak{a}}}
\providecommand{\frakb}{\ensuremath{\mathfrak{b}}}
\providecommand{\frakc}{\ensuremath{\mathfrak{c}}}
\providecommand{\frakd}{\ensuremath{\mathfrak{d}}}
\providecommand{\frake}{\ensuremath{\mathfrak{e}}}
\providecommand{\frakf}{\ensuremath{\mathfrak{f}}}
\providecommand{\frakg}{\ensuremath{\mathfrak{g}}}
\providecommand{\frakh}{\ensuremath{\mathfrak{h}}}
\providecommand{\fraki}{\ensuremath{\mathfrak{i}}}
\providecommand{\frakj}{\ensuremath{\mathfrak{j}}}
\providecommand{\frakk}{\ensuremath{\mathfrak{k}}}
\providecommand{\frakl}{\ensuremath{\mathfrak{l}}}
\providecommand{\frakm}{\ensuremath{\mathfrak{m}}}
\providecommand{\frakn}{\ensuremath{\mathfrak{n}}}
\providecommand{\frako}{\ensuremath{\mathfrak{o}}}
\providecommand{\frakp}{\ensuremath{\mathfrak{p}}}
\providecommand{\frakq}{\ensuremath{\mathfrak{q}}}
\providecommand{\frakr}{\ensuremath{\mathfrak{r}}}
\providecommand{\fraks}{\ensuremath{\mathfrak{s}}}
\providecommand{\frakt}{\ensuremath{\mathfrak{t}}}
\providecommand{\fraku}{\ensuremath{\mathfrak{u}}}
\providecommand{\frakv}{\ensuremath{\mathfrak{v}}}
\providecommand{\frakw}{\ensuremath{\mathfrak{w}}}
\providecommand{\frakx}{\ensuremath{\mathfrak{x}}}
\providecommand{\fraky}{\ensuremath{\mathfrak{y}}}
\providecommand{\frakz}{\ensuremath{\mathfrak{z}}}

%%%% Marker:defs from Yihui's cache %%%%
\def\01{\{0,1\}}
\newcommand{\eps}{\varepsilon}
%\newcommand{\veps}{\varepsilon}
%\newcommand{\al}{\ensuremath{\alpha}}
\newcommand{\C}{\ensuremath{\mathcal{C}}}
\newcommand{\D}{\ensuremath{\mathcal{D}}}
\newcommand{\F}{\ensuremath{\mathcal{F}}}
\newcommand{\G}{\ensuremath{\mathcal{G}}}
\newcommand{\K}{\ensuremath{\mathcal{K}}}
\newcommand{\mN}{\ensuremath{\mathcal{N}}}
\newcommand{\X}{\ensuremath{\mathcal{X}}}
\newcommand{\Y}{\ensuremath{\mathcal{Y}}}
\newcommand{\PAC}{\ensuremath{\mathsf{PAC}}}
%\newcommand{\id}{\ensuremath{\mathbb{I}}}
\newcommand{\eq}[1]{Eq.~\eqref{#1}}
\newcommand{\ineq}[1]{Ineq.~\eqref{#1}}
\newcommand{\Exp}{\mathbb{E}}
%\newcommand{\rank}{\mbox{\rm rank}}
%\newcommand{\tr}[1]{\Tr\left(#1\right)}

%%%%% Algorithms %%%%%%%%%
\newcommand{\Ord}[1]{\mathcal{O}\mleft( #1 \mright)}
\newcommand{\tOrd}[1]{\tilde{\mathcal{O}}\mleft( #1 \mright)}

%%%%% Bras and kets %%%%%%%%
%\newcommand{\bra}[1]{\langle{#1}|}
%\newcommand{\ket}[1]{|{#1}\rangle}
\newcommand{\brkt}[2]{\langle{#1}|{#2}\rangle}
%\newcommand{\ketbra}[2]{|{#1}\rangle\langle{#2}|}
\newcommand{\ketbraz}{\ketbra{0^a}{0^a}}

%%%% Typing absolute values %%%%%%%
%\DeclarePairedDelimiter\abs{\lvert}{\rvert}%
%\DeclarePairedDelimiter\norm{\lVert}{\rVert}%

% Swap the definition of \abs* and \norm*, so that \abs
% and \norm resizes the size of the brackets, and the 
% starred version does not.
\makeatletter
\let\oldabs\abs
\def\abs{\@ifstar{\oldabs}{\oldabs*}}
%
\let\oldnorm\norm
\def\norm{\@ifstar{\oldnorm}{\oldnorm*}}
\makeatother


